LensDFF: Language-enhanced Sparse Feature Distillation for Efficient Few-Shot Dexterous Manipulation

Learning dexterous manipulation from few-shot demonstrations is a significant yet challenging problem for advanced, human-like robotic systems. Dense distilled feature fields have addressed this challenge by distilling rich semantic features from 2D visual foundation models into the 3D domain. However, their reliance on neural rendering models such as Neural Radiance Fields (NeRF) or Gaussian Splatting results in high computational costs. In contrast, previous approaches based on sparse feature fields either suffer from inefficiencies due to multi-view dependencies and extensive training or lack sufficient grasp dexterity. To overcome these limitations, we propose Language-ENhanced Sparse Distilled Feature Field (LensDFF), which efficiently distills view-consistent 2D features onto 3D points using our novel language-enhanced feature fusion strategy, thereby enabling single-view few-shot generalization. Based on LensDFF, we further introduce a few-shot dexterous manipulation framework that integrates grasp primitives into the demonstrations to generate stable and highly dexterous grasps. Moreover, we present a real2sim grasp evaluation pipeline for efficient grasp assessment and hyperparameter tuning. Through extensive simulation experiments based on the real2sim pipeline and real-world experiments, our approach achieves competitive grasping performance, outperforming state-of-the-art approaches.

==> chapters/3_method_old.tex <==
\section{Method}
\subsection{Problem Formulation}
We assume a robot arm equipped with a dexterous \hand~ and a single eye-in-hand calibrated RGBD camera.  
A grasp $\mathbf{g} \in \mathbb{R}^d$ is represented by the 15-DOF hand joint configuration $\boldsymbol{j} \in \mathbb{R}^{15}$ and the 6D pose $(\mathbf{R},\mathbf{t}) \in SE(3)$ of the palm.

During the demo collection, the robot moves to 4 different poses where the object is visible to the camera. Each demo consists of a ground truth grasp pose $\mathbf{g_{gt}}$, a prompt describing the object $p$, point clouds $X_i$ and color image $I_i, i=[1,2,3,4] $ from $i_{th}$ view. During testing, the robot moves to one single pose to capture one camera observation given single or cluttered scenes. The task is to pick up the correct object given a language prompt that describes the target object.

\TODO{Add a paragraph to briefly introduce the pipeline with hyperlinks to subsections below}

\subsection{Grasp Demonstration with Primitives}

To endow our robotic system with dexterous manipulation capabilities from a limited set of real-world demonstrations, we employ five distinct grasp primitives: hook, cylindrical, pinch, tripod, and lumbrical grasps.
To endow our robotic system with dexterous manipulation capabilities from a limited set of real-world demonstrations, we employ five distinct grasp primitives: hook, cylindrical, pinch, tripod, and lumbrical grasps.
In each demonstration, a human expert selects the most suitable primitive for the task. Moreover, an object can be manipulated using multiple primitives; for example, when handling a cup, a pinch grasp is applied to the handle while a cylindrical grasp is used for the body (see Fig.~\ref{fig:demos} for details).

\begin{figure*}[htbp]
\vspace{10pt}
    \centering
    \includegraphics[width=0.8\textwidth]{materials/4_experiment/primitives_demos.pdf}
    \vspace{5pt}
    \caption{Demonstrating Diverse Grasp Primitives.
    This figure showcases the versatility of our collected demos using different primitives across a range of objects.
    (a) \textbf{Pinch grasp}: The robot delicately pinches the ear of the teddy bear between the thumb and index finger, demonstrating precision and control for manipulating small or delicate objects. 
    (b) \textbf{Hook grasp}: The robot employs a hook grasp to firmly hold the handle of the dustpan. This grasp utilizes the fingers to form hooks, securing the object for lifting or carrying.
    (c) \textbf{Tripod grasp}: The robot grasps the Mentos gum package using a tripod grasp, with the thumb and two fingers providing stability and dexterity for precise manipulation.
    (d) \textbf{Cylindrical grasp}: The robot encircles the body of the white mug with its fingers, forming a cylindrical grasp. This grasp configuration provides stability and force closure for larger objects.
    (e) \textbf{Lumbrical grasp}: The robot adopts a lumbrical grasp to hold the crackers box. In this grasp, the fingers are positioned parallel to the object's surface, offering a secure grip for flat or boxy objects.
    }
    \label{fig:demos}
\end{figure*}

% Apply CLIP for each view
% Given several camera observations from a demonstration, our approach first extracts features $F$ from every 2D image $I$. % onto 3D point clouds $X$ with pixel-point correspondences.


\subsection{Zero-Shot 3D Feature Distillation}
% CLIP background (This has to be deeper understood)
After demonstration collection, we first obtain the bbox and segmentation mask via SAM2~\cite{ravi2024sam2}, given the demonstration prompt. The bbox-cropped image will be sent to CLIP to extract vision features, where the segmentation mask is used to extract pixel-level features and corresponding 3D points.

A consistent and meaningful 3D features are essential to match with the test scene for robot manipulation. Current vision-language foundation models such as CLIP~\cite{radford2021clip} have demonstrated superior performance in extracting vision-language aligned features. However, they are aligned as a whole instead of pixel level, where a fine-grained alignment is missing~\cite{zhong2021regionclip}.
% cannot simple merge
Thus, simply merging the point clouds with projected vision features will result in view-inconsistent object surface 3D features due to a lack of 3D awareness in the 2D vision foundation model. 

To tackle this issue, in contrast to training an extra alignment network purely on vision features in~\cite{wang2024sparsedff}, an efficient language-enhanced zero-shot feature alignment is proposed, to adaptively align features cross views using language features from CLIP~\cite{radford2021clip}, where no extra training or finetuning is required.

% \textbf{Single View Pixel-aligned Features}
% Inspired by~\cite{jata2023conceptfusion}, the pixel-aligned features for the target objects detected with GroundedSAM~\cite{ren2024groundedsam}, 
% is computed with a weighted combination of global features $\mathbf{f}_{\text{vis}}^{G}$ and its local features $\mathbf{f}_{\text{vis}}^{L}$. The weight is obtained through the consine similarity between these two features. 


% \[
% \text{cos\_sim}(\mathbf{f}_{\text{vis}}^{G}, \mathbf{f}_{\text{vis}}^{L}) 
% \right\rangle 
% \;=\; \frac{\left(\mathbf{f}_{\text{vis}}^{L}\right)^{\mathsf{T}} \,\mathbf{f}_{\text{vis}}^{G}}
%        {\|\mathbf{f}_{\text{vis}}^{L}\|\;\|\mathbf{f}_{\text{vis}}^{G}\|\;+\;\epsilon}.
% \]

% \[ 
% w_i = \text{cos\_sim}(\mathbf{f}_{\text{vis}}^{G}, \mathbf{f}_{\text{vis}}^{L}) 
% \]


% where $\epsilon$ is used as a small value, e.g., $1e-8$ to avoid division by zero. Using the cosine similarity as the weight, we can compute the pixel-aligned vision local features:

% \[
% \mathbf{f}_{\text{vis}}^{\text{aligned}}
% \;=\;
% w_i\,\mathbf{f}_{\text{vis}}^{G}
% \;+\;
% \bigl(1 - w_i\bigr)\,\mathbf{f}_{\text{vis}}^{L}.
% \]

% \begin{figure}
% \vspace{5pt}
%     \centering
%     \includegraphics[width=0.4\textwidth]{materials/3_method/feature_aling.pdf}
%     \vspace{5pt}
%     \caption{Feature alignment}
%     \label{fig:robot_setup}
% \end{figure}

\textbf{Multi View Adaptive Language-aligned Features}

\begin{figure*}[htbp]
\vspace{10pt}
    \centering
    \includegraphics[width=\textwidth]{materials/3_method/feature_distill.pdf}
    \vspace{5pt}
    \caption{Multi View Adaptive Language-aligned Features
    \textbf{\color{red}add adaptive part for aligning demo/test object lan feat}}
    \label{fig:feature-distill}
\end{figure*}

Even though CLIP~\cite{radford2021clip} has inconsistent features across views, the language features are the same for our case, where the target objects exist through all views.

Given a demonstration prompt $p$ describing the object, we adaptively project CLIP vision features on every point $x_i$ into the corresponding language feature $\mathbf{f}_{lan}$ to obtain an aligned feature. The projected features are sent to the sigmoid activation function $\sigma$ for better normalization and interpretability.

\[
\mathbf{f}_i^{\text{aligned}}
= \sigma\!\Bigl(
   \frac{\langle \mathbf{f}_{\text{vis}}(x_i),\, \mathbf{f}_{\text{lan}} \rangle}
        {\|\mathbf{f}_{\text{lan}}\|^2}
\Bigr)\, \mathbf{f}_{\text{lan}}.
\]
During testing we found out the final grasp often doesn't work well if the demo object prompt features $\mathbf{f}_{\text{lan}}^{\text{demo}}$ differ a lot from test object prompt features $\mathbf{f}_{\text{lan}}^{\text{test}}$. Here we propose an adaptive language alignment strategy by comparing the cosine similarity between these two language features. If the cosine similarity is higher than a threshold, we use $\mathbf{f}_{\text{lan}}^{\text{demo}}$; otherwise, we use the fused language feature from both.

\[
s = \frac{\mathbf{f}_{\text{lan}}^{\text{demo}} \cdot \mathbf{f}_{\text{lan}}^{\text{test}}}
    {\|\mathbf{f}_{\text{lan}}^{\text{demo}}\| \|\mathbf{f}_{\text{lan}}^{\text{test}}\|}
\]
\[
\mathbf{f}_{\text{lan}} =
\begin{cases}
    \mathbf{f}_{\text{lan}}^{\text{demo}}, & \text{if } s \geq \tau, \\
    \frac{\mathbf{f}_{\text{lan}}^{\text{demo}} + \mathbf{f}_{\text{lan}}^{\text{test}}}{2}, 
    & \text{otherwise}.
\end{cases}
\]
here $\tau = 0.63$, after tuning with the real2sim evaluation, detailed in Section.~\ref{sec:real2sim}.

Unlike previous works of reconstructing a continuous features field using NeRF~\cite{mildenhall2020nerf} or Gaussian Splating\cite{kerbl20233dgaussiansplatt} where the grasp features can be computed by locating the grasp in 3D feature field.  
After distilling the features into 3D space, our grasp features $\mathbf{f}_{\text{grasp}}$ is computed by finding nearby 3D points $\mathbf{x}_i$ corresponding to hand surface points $q$ and aggregating their corresponding aligned features, weighted by the inverse of the L2 distance.

\[
\mathbf{f}_{\text{grasp}}
= \sum_{i=1}^{N} w_i \mathbf{f}_i^{\text{aligned}}
\quad\text{where}\quad
w_i 
= \frac{\frac{1}{\|\mathbf{q} - \mathbf{x}_i\|^2}}{\sum_{j=1}^{N} \frac{1}{\|\mathbf{q} - \mathbf{x}_j\|^2}}.
\]

This framework is applied both to demo and test RGBD images to extract multi-view consistent pixel-level 3D features, which will be utilized for grasp optimization.

% \subsection{Hierarchical Demo Retrieval}
% During test, we need to retrieve the proper grasp primitive and the optimal demonstration before grasp optimization.

% For an efficient demo retrieval, a hierarchical structure of grasp primitives and grasp demonstrations are depicted in {fig}.

% The retrieval first find the proper grasp primitive by computing the cosine similarity between the task prompt $p_t$ and a set of graps primitive prompts $p_k$, where $k \;\in\; \text{[hook, cylindrical, pinch, tripod and lumbrical]}$.

% \begin{align*}
% \text{cos\_sim}(\mathbf{p_t}, \mathbf{p}_k) 
% &= \frac{\mathbf{t} \cdot \mathbf{p}_k}{\|\mathbf{t}\|\;\|\mathbf{p}_k\|} \\ 
% k^* &= \arg\max_{k}\; \text{cos\_sim}(\mathbf{t}, \mathbf{p}_k)
% \end{align*}

\subsection{Primitive-based Grasp Sampler}

\textbf{Sampling palm poses} Given segmented target object point clouds, generating diverse and proper grasp poses is beneficial for a more efficient grasp optimization afterwards, especially given only single views of test objects.
The primitive-based grasp sampler first samples the palm poses and then joint configurations sequentially. 

A grasp frame is defined for \hand~ which is located at the center of the palm and oriented at middle of the thumb and index finger in Fig.\ref{fig:hand_frame} (a). First, The palm pose x-axis is encouraged to aim towards objects, so we choose point cloud normals to align the x-axis for every grasp sample. Afterwards, a 3D bounding box is aligned to the object point cloud, and the longer side is the y-axis. The sampled palm pose is perturbed with both translational and rotational noise. Just to note that in Fig.~\ref{fig:hand_frame} (c), given a single view point cloud, the point cloud normal direction can be ambiguous therefore, grasp samples exist on both sides of the object surface.

\begin{figure}[!h]
    \begin{adjustbox}{center}%{max width=1\linewidth}
    \centering
    \subfigure[Grasp frame]{
        \centering
        \includegraphics[width=0.22\columnwidth]{materials/3_method/hand_frame.png}
    }
    \subfigure[Sample from point cloud normal]{
        \centering
        \includegraphics[width=0.25\columnwidth]{materials/3_method/sampled_palm_pose.png}
    }
    \subfigure[Sampled poses]{
        \centering
        \includegraphics[width=0.4\columnwidth]{materials/3_method/drill_heuristic.png}
    }
    \end{adjustbox}
    \caption{Visualization of the palm pose sampling}
    \vspace{-1em}
    \label{fig:hand_frame}
\end{figure}

\textbf{Sampling primitive-based joint configurations}
% Random sampling is stupid
For each grasp primitive, there is a corresponding eigengrasp~\cite{ciocarlie2009hand}, which reduces the dimension of the search space for the sampling process. 

Taking pinch grasp as an example, only the index and thumb are closing, thus their eigengrasp controls the index and thumb with same commands. Similarly, the cylindral grasp closes every finger so their eigengrasp. The initial joint configurations are sampled given the designed eigengrasp for each grasp primitive. 

% Instead, we build upon the idea from Ciocarlie \cite{ciocarlie2009hand} to sample in a meaningful subspace spanned by the so-called \textit{eigengrasps}.
% % Explain where the idea came from
% % Ciocarlie's work was inspired by the Neuroscience community, which showed that the joint DoFs of human hands during real-world grasping trials were largely not operating independently but coordinated. More than 80 \% of the variation in the data could be explained from the two first components of the principal component analysis (PCA).
% % What are eigengrasps
% % These components were termed eigengrasps as almost any grasp joint configuration can be synthesized as of linear combination of a few eigengrasps. 
% % Obtaining eigengrasps
% We manually define four eigengrasps $\mathbf{e_1}, \mathbf{e_2}, \mathbf{e_3}, \mathbf{e_4} \in \mathbb{R}^{15}$. The full joint configuration:
% \vspace{-1em}
% \begin{equation}
%     \mathbf{\theta} = \sum_{i=1}^4 \alpha_i \mathbf{e}_i
% \end{equation}
% % Just sample coefficient
% is obtained through sampling the coefficients $\alpha_i\in[0,1]$.


\subsection{Grasp Optimization}
The grasp pose $\textbf{g}$ is optimized given initial grasp generated from the grasp sample and the following optimization process.

The optimization objective is to minimize the difference between the grasp features $\textbf{f}_{\text{grasp}}$ from the demo scene and those from the test scene.
To avoid potential self-collision, additionally, a self-penetration energy function~\cite{wang2023dexgraspnet} is added to the optimization. Additionally, a normal direction restriction is applied where the final pose should not too deviate from the initial pose sampled from the point cloud's normal direction.
\[
E_{\text{feat}}(\mathbf{g}) = \left\lVert \mathbf{f}_{\text{grasp}}^{\text{demo}}
      \;-\; 
      \mathbf{f}_{\text{grasp}}^{\text{test}}(\textbf{g})
      \right\rVert^2
\]

\[
\min_{\textbf{g}}\; E(\textbf{g})
\;=\;
\underbrace{E_{\text{feat}}(\mathbf{g})}_{\text{feature diff.}}
\;+\;
\underbrace{\lambda_{\text{spen}} \, E_{\text{spen}}(\textbf{g})}_{\text{self-penetration}}
\;+\;
\underbrace{\lambda_{\text{normal}} \, E_{\text{normal}}(\textbf{g})}_{\text{normal restriction}}
\]
here $\lambda_{\text{normal}}$ and $\lambda_{\text{spen}}$ are $1e-2$.

Unlike the Shadow Hand used in~\cite{wang2023dexgraspnet}, penalizing hand-object penetration is not recommended in our setup because our hand uses an impedance controller in which the target joints typically penetrate the objects in order to apply sufficient contact force. Therefore, we exclude this term from the optimization. 


